Analysis of Attacker Behavior in Compromised Hosts During Command and Control

Traditional reactive approach of blacklisting botnets fails to adapt to the rapidly evolving landscape of cyberattacks. An automated and proactive approach to detect and block botnet hosts will immensely benefit the industry. Behavioral analysis of botnet is shown to be effective against a wide variety of attack types. Current works, however, focus solely on analyzing network traffic from and to the bots. In this work we take a different approach of analyzing the chain of commands input by attackers in a compromised host. We have deployed several honeypots to simulate Linux shells and allowed attackers access to the shells to collect a large dataset of commands. We have further developed an automated mechanism to analyze these data. For the automation we have developed a system called CYbersecurity information Exchange with Privacy (CYBEX-P). Finally, we have done a sequential analysis on the dataset to show that we can successfully predict attacker behavior from the shell commands without analyzing network traffic like previous works.

==> 3-background.tex <==


\section{Background}\label{sec:back}

\subsection{Honeypot}

An honeypot is a decoy system. The Honeynet project \cite{spitzner2003honeynet} defines an honeypot as \textit{A security resource who’s value lies in being probed, attacked or compromised}. As honeypots have no production value, any activity logged in an honeypot can be deemed malicious.

Honeypots can be classified into two categories based on their purpose:

\begin{enumerate}
    \item Production honeypot: Production honeypots are used in campus networks to lure attackers away from production machines. They can also be used to detect attacker IP addresses or email addresses. They protect production servers by posing themselves easy targets for attackers.

    \item Research honeypot: Research honeypots are used to collect information. This information is further analyzed to detect new tools and techniques, to understand behavior of attackers and to detect attack patterns. Finally, the analyzed data can lead to newer defense techniques.
\end{enumerate}


Honeypots can be further classified into three categories on their level of interaction with the attacker:

\begin{enumerate}
    \item High Interaction Honeypots: Simulates all aspects of a real operating system (OS) completely. These honeypots can collect more information. However they are more risky to maintain, because the attacker can launch further attacks from these.
    \item Medium Interaction Honeypots: Simulates the aspects of an OS which cannot be used to launch further attacks.
    \item Low Interaction Honeypots: Simulates very basic aspects of an OS. They can collect very limited information and are low risk.
\end{enumerate}


\subsection{Cowrie Honeypot}

Cowrie \cite{oosterhof2016cowrie} is a medium to high interaction SSH and Telnet honeypot designed to log brute force attacks and the shell interaction performed by the attacker. In medium interaction mode (shell) it emulates a UNIX system in Python, in high interaction mode (proxy) it functions as an SSH and telnet proxy to observe attacker behavior to another system. In this work we use Cowrie in the medium interaction mode.

In our setup, cowrie only allows SSH logins into our honeypot. An attacker can login to the system using any username and password combination. Cowrie logs all the interactions including the source IP address of the attacker, the SSH parameters and the commands input while the attacker is logged in.

\subsection{Mirai Botnet}

Mirai consists of a family of malware used to hijack poorly protected IoT devices. This botnet (or its derivatives) poses a major threat to the IoT landscape. It can be used to perform large scale DDoS attacks of bitcoin mining. Mirai connects to random public IP address and performs Telnet or SSH scanning. If the connection succeeds, it tries to login into the shell using common username and passwords from a table. If the login is successful, Mirai downloads and runs bot binaries into the device. It then repeats the process using the new bot. Mirai has seen unprecedented spread due to the large number of poorly protected IoT devices on the internet.

\subsection{CYBEX-P}

CYbersecurity Information Exchange with Privacy (CYBEX-P) \cite{sadique2019system} is a cybersecurity information sharing (CIS) platform with robust data governance. It automatically analyzes shared data to generate insightful reports and alerts. CYBEX-P has builtin software modules for data collection, data storage, data analysis and report generation. In this work we use CYBEX-P infrastructure as a service (IaaS) for collecting and analyzing the honeypot data.

